Optimum Configuration for Hovering n-Quadrotors carrying a Slung Payload

This work proposes a strategy for organising quadrotors around a payload to enable hovering without external stimuli, together with a MATLAB software for modelling the dynamics of a quadrotor-payload system. Based on geometric concepts, the proposed design keeps the payload and system centre of mass aligned. Hovering tests that are successful confirm the method's efficiency. Moreover, the algorithm is improved to take thrust capacities and propeller distances into account, calculating the minimum number of quadrotors needed for hovering. The algorithm's effectiveness is demonstrated by numerical examples, which reveal that larger quadrotors may require fewer units while smaller ones give greater flexibility. Our code can be found at: \href{https://github.com/Hosnooo/Swarm-Slung-Payload}{https://github.com/Hosnooo/Swarm-Slung-Payload}

==> Sections/Methodology.tex <==

% \section{ (n) Quadrotors}
% For n quadrotors, let us define  \begin{equation}
%   \mathbf{\digamma} = \begin{bmatrix}
%     I_3 \dots & I_3 \\
%     \hat{\mathbf{\rho}}_1  \dots & \hat{\mathbf{\rho}}_n
%     \end{bmatrix}   
%   \label{eq: BIGrho}
% \end{equation}


% $\mathbf{\digamma} \text{ is assumed to be of rank } \geq 6$ to ensure that the degrees of freedom are enough for controlling the translational and rotational motion. This indicates that the number of drones $\mathbf \geq 3 $ to be able to control the drone attitude and rotate it along three axes.

% The desired trajectory for the payload's attitude and position is assumed to be given as \begin{equation} R_{0d} = R_{0d}\times \hat\Omega_{0d}. \label{equation}\end{equation}
% where $\Omega_{0d} \in R^3$ is the desired angular rate. In this section we follow \cite{lee2014geometric1} to construct a geometric controller, namely $f_i$ and $M_i$ that makes the zero trajectory errors state asymptotically stable. 

% Since the parallel component of $u_i$ affects payload motion and the perpendicular component affects link motion, the $\mathbf{u}_{\parallel \mathbf{i}}$ is designed first for the payload to follow the desired trajectory, followed by the $\mathbf{u}_{\perp \mathbf{i}}$ design to determine the orientation of the links.

% Considering $a_i \in R^3$ as the acceleration of the point of payload that is connected to link,it is defined as: \begin{equation}
% a_i = \Ddot{x_0}-g\times e_3 + R_0 \times \hat\Omega_0^2 \times{\mathbf{\rho}} -R_0 \times \hat{\mathbf{\rho}} \times \dot\Omega_0. \label{eq:a_i}
% \end{equation}
% The parallel component of the control input is chosen as:

% \begin{equation}
%     u_i^{\parallel} = \mu_i +m_i l_i \norm{\omega}_i q_i + m_i q_i q_i^T  a_i
% \label{eq: desired_final_ui_para}
% \end{equation}

% $\mu_i \in R^3$ is considered as a virtual control input and is evident to be parallel to ${q}_i$.

% substituting back equation (13) in equations (1) and (2), we get\begin{equation}
% m_0 (\Ddot{x_0}- ge_3) = \sum_{i=1}^{n} \mu_i
% \label{eq:mu_F}
% \end{equation}

% \begin{equation}
%     J_0 \Dot{\Omega_0} + \hat\Omega_0 J_0 \Omega_0 = \sum_{i=1}^{n} \hat\rho_i R_0^T \mu_i
%     \label{equ:mu_J0}
% \end{equation}
% It is clear that $\mu_i$ represents force on payload from link of each drone. Substituting equation (\ref{eq:mu_F})  and (\ref{equ:mu_J0}), back into (\ref{eq:a_i}).
% \begin{equation}
% a_i = \frac{1}{m_0} \sum_{j=1}^{n} \mu_j + R_0 \hat\Omega^ 2  \rho_i + R_0 \hat\rho J_0^{-1} 0 (\hat\Omega_0 J_0 \Omega_0 - \sum_{j=1}^{n} \hat\rho_j R^T_0 \mu_j )
% \label{eq:final a_I}
% \end{equation}

% We implement a nonlinear controller of proportional-derivative type for control. The positional, angular velocity, and attitude tracking errors are characterized as follows:

% \begin{equation}
% \mathbf{e}_{x_0} = x_0 - x_{0_d}, 
% \label{eq:track_X_0}
% \end{equation}

% \begin{equation}
% \mathbf{e}_{R_0} = \frac{1}{2} \left( R_{0_d}^T R_{0} - R_0^T R_{0_d} \right)^\vee, 
% \label{eq:track_R0}
% \end{equation}

% \begin{equation}
% \mathbf{e}_{\Omega_0} = \Omega_0 - R_0^T R_{0_d} \Omega_{0_d}.
% \label{eq:track_Omega_0}
% \end{equation}

% Next is getting the $F_d$ and $M_d$ defined in terms of tracking errors 

% \begin{equation}
% F_d = m_0(-k_{x_0} \mathbf{e}_{x_0} - k_{\dot{x}_0} \dot{\mathbf{e}}_{x_0} + \ddot{x}_{0_d} - g\mathbf{e}_3), \quad 
% \label{eq:F_desired}
% \end{equation}

% \begin{equation}
% M_d = -k_{R_0}\mathbf{e}_{R_0} - k_{\Omega_0}\mathbf{e}_{\Omega_0} + (R_0^T R_{0d} \Omega_{0d})^\vee J_0 R_0^T R_{0_d} \Omega_{0_d} + J_0 R_0^T R_{0_d} \dot{\Omega}_{0_d}
% \label{eq:M_desired}
% \end{equation}
% Where the coefficients $k_{x_0}, k_{\dot{x_0}} , k_{R_0}, k_{\Omega_0} \in R.$ are positive.

% Now, we get $\mu_d$ defined through $F_d$ and $M_d$ through the matrix $\mathbf{\digamma}$, as it guarantees the existence of at least one unique solution. Hence using least squares minimum-norm solution, we get 
% \begin{equation}
% \begin{bmatrix}
% R_0^T \mu_{1d} \\
% \vdots \\
% R_0^T \mu_{nd}
% \end{bmatrix}
% =
% \begin{bmatrix}
% R_0^T F_d \\
% M_d
% \end{bmatrix}
% \label{eq: F_d+M_d}
% \end{equation}

% \begin{equation}
% \begin{bmatrix}
% \mu_{1d} \\
% \vdots \\
% \mu_{nd}
% \end{bmatrix}
% =\text{diag}[R_0, \dots, R_0] P^T (PP^T)^{-1} \begin{bmatrix} R_0^T F_d \\ M_d
% \end{bmatrix}
% \label{eq:mU_d}
% \end{equation}
% This structure will not violate the condition for $\mu_i$ to be parallel to $q_i$ as it is given by 
% \begin{equation}
% \mu_i = (\mu_{id} \cdot q_i) q_i = q_i q_i^T \mu_{id}
% \label{eq: mu_i->mu_d}
% \end{equation}
% and the desired orientation of each link is 

% \begin{equation}
% q_{i_d} = -\frac{\mu_{i_d}}{\lVert \mu_{i_d} \rVert}.
% \label{eq:final q_d}
% \end{equation}
% When $q_i$ is equal to $q_{i_d}$, $F_i$, and $M_i$ will go to $F_d$ and $M_d$. Now for designing perpendicular component of $u_i$, substitute equation (\ref{eq: desired_final_ui_para}) in equation (\ref{eqn:omega_i}).
% \begin{equation}
% \dot{\omega}_i = \frac{1}{l_i} \hat{q}_i a_i - \frac{1}{m_i l_i} \hat{q}_i u_{ i}^\perp.
% \end{equation}

% It is desired to get $w_i$ so that $q_i$ converge to $q_{i_d}$. Hence by using equation (\ref{eqn:q_i}) and arranging it we get that
% \begin{equation}
% \omega_{i_d} = q_{i_d} \times \dot{q}_{i_d} 
% \label{eq:desired_w_i}
% \end{equation}

% and the tracking error, and $u_i^\perp$ accordingly are defined as 
% \begin{equation}
% \mathbf{e}_{q_i} = q_{i_d} \times q_i,
% \label{eq:track_q}
% \end{equation}
% \begin{equation}
% \mathbf{e}_{{\omega}_i} = \omega_i + \hat{q}_i^2 \omega_{i_d}, 
% \label{eq:track_w_i}
% \end{equation}

% \begin{equation}
% u_{i}^\perp  = m_i l_i \hat{q}_i \left( -k_q \mathbf{e}_{q_i} - k_{\omega} \mathbf{e}_{\omega_i} - (\mathbf{q}_i \cdot \omega_{i_d}) \dot{\mathbf{q}}_i - \hat{q}_i^2 \dot{\omega}_d \right) - m_i \hat{q}_i^2 a_i
% \label{eq: final desired _ui_perp}
% \end{equation}

% where $k_q$,$k_w$ are positive constants. Substituting the expression of $u_{i}^\perp$ back into (\ref{eq:desired_w_i})
% \begin{equation}
%  \dot{\omega}_i = -k_q \mathbf{e}_{q_i}- k_{\omega} \mathbf{e}_{\omega_i} - (\mathbf{q}_i \cdot \dot{\omega}_{i_d}) \dot{\mathbf{q}}_i - \hat{q}_i^2 \dot{\omega}_d.
%  \label{eq:final desired wi}
% \end{equation}

% However, since  $u_i$ needs to be in third body axis , The magnitude of thrust is determined by the projection of $u_i$ onto - $R_ie_3$
% the force that is be applied to achieve the desired trajectory.

% \begin{equation}
%     f_i=-u_i \cdot(R_I e_3)
%     \label{eq: final desired fi}
% \end{equation}

% Consequently , the desired trajectory is achieved if third body axis, namely $b_3$ $\in s^2$ for each quad rotor is  parallel to the desired $u_i$, 
% \begin{equation}
% b_{3_i} =-\frac{u_i}{\norm{u_i}}
% \label{eq: b_3}
% \end{equation}
% This will impose a two-dimensional constraint on quad rotor attitude, where $b_{1_i}$  should be perpendicular on the third axis. Hence defining $b_{1_i} \in s^2$ to be a smooth function in time as 
% \begin{equation}
% b_{1_i}= - \frac{(\hat{b}_{3i})^2 \mathbf{b}_{1i}}{\lVert (\hat{b}_{3i})^2 \mathbf{b}_{1_i} \rVert}
% \label{eq:b_1}
% \end{equation}
% and $b_{2_i} \in s^2$  is orthogonal to the two vectors resulting in desired rotation matrix for each drone to be 
% \begin{equation}
% R_{i_c} = \left[ - \frac{(\hat{b}_{3_i})^2 \mathbf{b}_{1_i}}{\lVert (\hat{b}_{3_i})^2 \mathbf{b}_{1_i} \rVert}, \frac{\hat{b}_{3_i} \mathbf{b}_{1_i}}{\lVert \hat{b}_{3_i} \mathbf{b}_{1_i} \rVert}, \mathbf{b}_{3_i} \right]
% \label{eq:final desired R drones}
% \end{equation}
% From equation(\ref{eqn: R_i}) we define the desired angular velocity 
% \begin{equation}
%     \Omega_{i_c} = (R_{i_c}^T \dot{R}_{i_c})^\vee
%     \label{eq:final desired omega drone}
% \end{equation}

% The tracking error for the quad rotor attitude and angular velocity is then designed as 

% \begin{equation}
%     e_{R_i} = \frac{1}{2} \left( R_{i_c}^T R_i - R_i^T R_{i_c} \right)^\vee, \quad e_{\Omega _i} = \Omega_i - R_i^T R_{i_c} \Omega_{i_c}.
%     \label{track_rotation-drone}
% \end{equation}
% The control moment is selected as a tracking controller utilizing the tracking error on $ \mathfrak{so}(3) $
% \begin{equation}
% M_i = -\frac{k_R}{\epsilon^2} e_{R_i} - \frac{k_\Omega}{\epsilon} e_{\Omega_ i} + \Omega_i \times J_i \Omega_i - J_i(\hat\Omega_i {R}_i^T R_{i_c}\Omega_{i_c} - R_i^T R_{i_c}\dot\Omega_{i_c})
% \label{Final desired moment }
% \end{equation} 

% ${k_R},{k_\Omega},\epsilon$ are positive constants.
% The algorithm adopted here is for a given desired $x_0, R_{0_d}$, a desired $b_{1_i}$ for each drone and control inputs $F_i$ , $ M_i$  constructed as in equations (\ref{eq: final desired fi}),  (\ref{Final desired moment } respectively, the tracking errors  $ {e}_{x_0} \dot{e}_{x_0}, e_{R_0}, e_{\Omega_0}, e_{q_i}, e_{\omega_i}, e_{R_i}, e_{\Omega_i}$ will have zero equilibrium that is exponentially stable.

\subsection{ (1) Quadrotor}
In this section, we consider a quadrotor with no payload. First, the equations of motion are as follows:
\begin{equation}
\dot{x} = v
\end{equation}
\begin{equation}
m\dot{v} = mg\mathbf{e}_3 - fR\mathbf{e}_3
\end{equation}

\begin{equation}
\dot{R} = R\hat{\Omega}
\end{equation}

\begin{equation}
J\dot{\Omega} + \Omega \times J\Omega = M
\end{equation}

For a given desired trajectory $x_d$, and desired direction of the first body-fixed axis $b_{1_d}$, the required rotation matrix becomes as follows 
\begin{equation}
\mathbf{R}_d = \begin{bmatrix}
{\mathbf{b}}_{2_d} \times {\mathbf{b}}_{3_d} &
{\mathbf{b}}_{2_d} &
{\mathbf{b}}_{3_d}
\end{bmatrix} \in SO(3),    
\end{equation}
where $b_{2_d}=\frac{{b}_{3_d} \times {b}_{1_d}}{\lVert {b}_{3_d} \times {b}_{1_d}\rVert}$
\\
\\

We implement a nonlinear controller of proportional-derivative type for control. The position, velocity, angular velocity, and attitude tracking errors are characterized as follows:

\begin{equation}
\mathbf{e}_{x} = x - x_d, 
\label{eq:track_X_0}
\end{equation}

\begin{equation}
 \mathbf{e}_v = \mathbf{v} - \mathbf{v}_d.  
\end{equation}

\begin{equation}
\mathbf{e}_{R} = \frac{1}{2} \left( R_{d}^T R- R^T R_{d} \right)^\vee, 
\label{eq:track_R}
\end{equation}

\begin{equation}
\mathbf{e}_{\Omega} = \Omega - R^T R_{d} \Omega_{d}.
\label{eq:track_Omega_0}
\end{equation}

An error function is defined on SO(3) as $
\Psi(R, R_d) = \frac{1}{2} \text{tr}(I - R_d^T R)$ and if rotation matrix changes by $\delta R = R\hat\eta  \text{ for } \eta \in \mathbb{R}^3.$ its derivative  is given by 
\begin{equation}
\frac{d}{dR} \Psi(R, R_d) \cdot R\hat\eta = -\frac{1}{2} \text{tr}(R_d^T R\hat\eta) = \frac{1}{2} ((R_d^T R - R^T R_d)^\vee \cdot \eta)
\end{equation}

Hence the tracking controller design is given by specifying the third body axis, and the forces and moments as 
\begin{equation}
   {b}_{3_d} = -\frac{(-k_x \mathbf{e}_x - k_v \mathbf{e}_v - mg\mathbf{e}_3 + m{\Ddot{x_d}})}
{\lVert(-k_x \mathbf{e}_x - k_v \mathbf{e}_v - mg\mathbf{e}_3 + m{\Ddot{x_d}}) \rVert}
\end{equation}

\begin{equation}
    f = -(-k_x\mathbf{e}_x - k_v\mathbf{e}_v - mg\mathbf{e}_3 + m{\Ddot{x_d}}) \cdot R\mathbf{e}_3
\end{equation}
\begin{equation}
 M = -k_R e_R - k_{\Omega}e_{\Omega} + \Omega \times J\Omega - J(\Omega^\wedge R^T R_d\Omega_d - R^T R_d\dot{\Omega}_d)
\end{equation}
It is assumed that the torque generated by each propeller is directly proportional to its thrust. From propeller configuration, the first and the third propellers rotate clockwise, and the second and the fourth propellers rotate counterclockwise, the torque generated by the $i$-th propeller can be written $T_i =(-1)^i c_{\tau f} f_i$. Hence, the force and moments are described by


\begin{equation}
\begin{bmatrix}
f \\
M_1 \\
M_2 \\
M_3
\end{bmatrix}
=
\begin{bmatrix}
1 & 1 & 1 & 1 \\
0 & -d & 0 & d \\
d & 0 & -d & 0 \\
-c_{\tau f} & c_{\tau f} & -c_{\tau f} & c_{\tau f}
\end{bmatrix}
\begin{bmatrix}
f_1 \\
f_2 \\
f_3 \\
f_4
\end{bmatrix}
\end{equation}



